LLM-DetectAIve: a Tool for Fine-Grained Machine-Generated Text Detection

The ease of access to large language models (LLMs) has enabled a widespread of machine-generated texts, and now it is often hard to tell whether a piece of text was human-written or machine-generated. This raises concerns about potential misuse, particularly within educational and academic domains. Thus, it is important to develop practical systems that can automate the process. Here, we present one such system, LLM-DetectAIve, designed for fine-grained detection. Unlike most previous work on machine-generated text detection, which focused on binary classification, LLM-DetectAIve supports four categories: (i) human-written, (ii) machine-generated, (iii) machine-written, then machine-humanized, and (iv) human-written, then machine-polished. Category (iii) aims to detect attempts to obfuscate the fact that a text was machine-generated, while category (iv) looks for cases where the LLM was used to polish a human-written text, which is typically acceptable in academic writing, but not in education. Our experiments show that LLM-DetectAIve can effectively identify the above four categories, which makes it a potentially useful tool in education, academia, and other domains. LLM-DetectAIve is publicly accessible at https://github.com/mbzuai-nlp/LLM-DetectAIve. The video describing our system is available at https://youtu.be/E8eT_bE7k8c.

==> emnlp2024-demo/section/demo_paper_guideline.tex <==
Submission Guidelines:
Link:  https://2024.emnlp.org/calls/demos/

Here are some things to make sure of when writing the paper, you can also look at the link above for extra info:

Main content
1. Maximum: 6 pages
2. with 2 pages for Appendix

According to the requirement above, we need:
1. a 2.5 mins video, upload to youtube and provide link
2. live demo website (ours are in huggingface)
3. a link to a downloadable installation package (github)



What problem does the proposed system address?
Why is the system important and what is its impact?
What is the novelty in the approach/technology on which this system is based?
Who is the target audience?
How does the system work?
How does it compare with existing systems?
How is the system licensed?
How was the system evaluated? Were user studies/human evaluation experiments conducted?
Note that this year, submissions that do not report any form of evaluation may be desk rejected.A Demonstration Video


A short (at most 2.5 minutes) screencast video demonstrating the system together with your paper submission. This screencast will be used to evaluate the paper, but won’t be published unless requested. For demos that can be presented on a screen, a screencast with audio narration is the most suitable format. If this is not feasible, a video showcasing user interaction with the system may be utilized. Production quality is not a priority, so we encourage to simply create a screencast of the software being demoed with minimal to no editing. We encourage publishing your video on YouTube or a similar site and including the link in your paper. If you prefer not to upload the video publicly, please submit it as supplementary material in MPEG4 format when you submit your paper through the official website.

Live Demo Website or Installable Package

A link to a live demo website; or a link to a downloadable installation package of the demo. Note that this is a strict requirement enforced this year, and submissions that do not provide links will be desk rejected. Exceptions will be made only in cases where sharing a link is clearly impossible, such as when special hardware is required. In such cases, authors must clearly state why a link cannot be provided.



